The population of Young Stellar Clusters throughout the disk of M33

The properties of young stellar clusters (YSCs) in M33, identified from the center out to about twice the size of the bright star-forming disk,are investigated. We find 915 discrete MIR sources as far as the extent of the warped HI disk, i.e. 16 kpc from the galaxy center. Their surface density has a steep radial decline beyond 4.5 kpc, and flattens out beyond the optical radius at 8.5 kpc. We are able to identify YSCs out to 12 kpc. At large galactocentric radii, the paucity of very luminous clusters and the relevance of hot dust emission become evident from the analysis of the bolometric and MIR luminosity functions. The YSC mass and size are correlated with a log-log slope of 2.09, similar to that measured for giant molecular clouds in M33 and the Milky Way, which represent the protocluster environment. Most of the YSCs in our sample have low extinction and ages between 3 and 10 Myr. In the inner regions of M33 the clusters span a wide range of mass (10^2<M<3 10^5 msun) and luminosity 10^38<L{bol}<3 10^{41}erg/s, while at galactocentric radii larger than 4 kpc we find a deficiency of massive clusters. Beyond 7 kpc, where the Halpha surface brightness drops significantly, the dominant YSC population has M<10^3 msun and a slightly older age (10 Myrs). This implies the occurrence of star formation events about 10 Myr ago as far as 10-12 kpc from the center of M33. The cluster L{FUV}--L{Halpha} relation is non-linear for L{FUV}<10^{39}erg/s, in agreement with randomly sampled models of the IMF which, furthermore, shows no appreciable variation throughout the M33 disk.

==> abstract.tex <==
The properties of young stellar clusters (YSCs) in M33, identified from the center out to about twice the size of the bright star-forming disk,are investigated. We find 915 discrete MIR sources as far as the extent of the warped HI disk, i.e. 16 kpc from the galaxy center. Their surface density has a steep radial decline beyond 4.5 kpc, and flattens out beyond the optical radius at 8.5 kpc. We are able to identify YSCs out to 12~kpc. At large galactocentric radii, the paucity of very luminous clusters and the relevance of hot dust emission become evident from the analysis of the bolometric and MIR luminosity functions. The YSC mass and size are correlated with a log-log slope of 2.09, similar to that measured for giant molecular clouds in M33 and the Milky Way, which represent the protocluster environment. Most of the YSCs in our sample have low extinction and ages between 3 and 10 Myr. In the inner regions of M33 the clusters span a wide range of mass (10^2<M<3 10^5 msun) and luminosity 10^38<L{bol}<3 10^{41}erg/s, while at galactocentric radii larger than 4 kpc we find a deficiency of massive clusters. Beyond 7 kpc, where the Halpha surface brightness drops significantly, the dominant YSC population has M<10^3 msun and a slightly older age (10 Myrs). This implies the occurrence of star formation events about 10 Myr ago as far as 10-12 kpc from the center of M33. The cluster L{FUV}--L{Halpha} relation is non-linear for L{FUV}<10^{39}erg/s, in agreement with randomly sampled models of the IMF which, furthermore, shows no appreciable variation throughout the M33 disk.
